Evaluating Search System Explainability with Psychometrics and Crowdsourcing

As information retrieval (IR) systems, such as search engines and conversational agents, become ubiquitous in various domains, the need for transparent and explainable systems grows to ensure accountability, fairness, and unbiased results. Despite recent advances in explainable AI and IR techniques, there is no consensus on the definition of explainability. Existing approaches often treat it as a singular notion, disregarding the multidimensional definition postulated in the literature. In this paper, we use psychometrics and crowdsourcing to identify human-centered factors of explainability in Web search systems and introduce SSE (Search System Explainability), an evaluation metric for explainable IR (XIR) search systems. In a crowdsourced user study, we demonstrate SSE's ability to distinguish between explainable and non-explainable systems, showing that systems with higher scores indeed indicate greater interpretability. We hope that aside from these concrete contributions to XIR, this line of work will serve as a blueprint for similar explainability evaluation efforts in other domains of machine learning and natural language processing.

==> figures/interface_b.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/rel_uncertain_b.jpg}
    \caption{Search interface shown to Group B (modeled on the basis of the system presented by Cohen et al. \citep{cohen2021not}). On the left-hand side, the two columns show a hypothetical relevance and confidence score for each result. The relevance score refers to how relevant the corresponding article is to the query. The confidence score refers to how confident the search engine is that it calculated the relevance score correctly.}
\end{figure}
    
\label{fig:interface_b}

==> figures/interface_c.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/baseline_c.jpg}
    \caption{Search interface shown to Group C. This interface served as our baseline as an example of a system with limited explainable elements.}
\end{figure}

\label{fig:interface_c}

==> figures/tlx_native.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.35\textwidth]{figures/tlx-resp-by-eng.jpg}
    \caption{NASA-RTLX responses between native (n=51) and non-native (n=49) English speakers. While non-native English speakers have a higher perceived task load than native English speakers on 3 dimensions, they had a lower perceived \textit{Temporal Demand} and \textit{Effort} for a higher perceived \textit{Performance}.}
    \label{fig:tlx-native}
% \vspace{-1.25em}
\end{figure}

==> tables/cfa_loadings.tex <==
\begin{table}[]
    \caption{Final factor loadings}
    \centering
    \begin{tabular}{cccc}
        \toprule
        \begin{tabular}[c]{@{}c@{}}Factors \&\\Items\end{tabular} & Original Factor Label & \begin{tabular}[c]{@{}c@{}}Std.\\Loading\end{tabular} & \begin{tabular}[c]{@{}c@{}}Std.\\Error\end{tabular}  \\ 
        \midrule
        \textbf{Factor 1} &  & 0.997 & 0.000 \\
        41 & Plausibility & 0.905 & 0.096 \\
        49 & Justifiability & 0.888 & 0.097 \\
        47 & Trustworthiness & 0.878 & 0.096 \\
        21 & Informativeness & 0.868 & 0.094 \\
        37 & Acceptability & 0.851 & 0.110 \\
        19 & Understandability & 0.825 & 0.087 \\
        15 & Transferability & 0.703 & 0.000 \\
        \textbf{Factor 2} &  & -0.944 & 0.065 \\
        2 & Decomposability & 0.938 & 0.094 \\
        22 & Global Interpretability & 0.928 & 0.098 \\
        24 & Local Interpretability & 0.921 & 0.098 \\
        0 & Simultability & 0.911 & 0.099 \\
        38 & Faithfulness & 0.894 & 0.097 \\
        4 & Algorithmic Transparency & 0.884 & 0.097 \\
        46 & Trustworthiness & 0.877 & 0.091\\
        6 & Causality & 0.842 & 0.095\\
        8 & Uncertainty & 0.792 & 0.092\\
        34 & Units of Explanation & 0.789 & 0.094 \\
        12 & Visibility & 0.723 & 0.092 \\        
        26 & Counterfactuals & 0.704 & 0.000 \\
        \bottomrule
    \end{tabular}
\label{tab:cfa_loadings}
\end{table}

